Measurement of the azimuthal anisotropy of charged particles produced in $\sqrt{s_\mathrm{NN}} = 5.02$ TeV Pb+Pb collisions with the ATLAS detector

Measurements of the azimuthal anisotropy in lead-lead collisions at $\sqrt{s_\mathrm{NN}} = 5.02$ TeV are presented using a data sample corresponding to 0.49 $\mathrm{nb}^{-1}$ integrated luminosity collected by the ATLAS experiment at the LHC in 2015. The recorded minimum-bias sample is enhanced by triggers for "ultra-central" collisions, providing an opportunity to perform detailed study of flow harmonics in the regime where the initial state is dominated by fluctuations. The anisotropy of the charged-particle azimuthal angle distributions is characterized by the Fourier coefficients, $v_{2}-v_{7}$, which are measured using the two-particle correlation, scalar-product and event-plane methods. The goal of the paper is to provide measurements of the differential as well as integrated flow harmonics $v_{n}$ over wide ranges of the transverse momentum, 0.5 $<p_{\mathrm{T}}<$ 60 GeV, the pseudorapidity, $|\eta|<$ 2.5, and the collision centrality $0-80$%. Results from different methods are compared and discussed in the context of previous and recent measurements in Pb+Pb collisions at $\sqrt{s_\mathrm{NN}} = 2.76$ TeV and 5.02 TeV. In particular, the shape of the $p_{\mathrm{T}}$ dependence of elliptic or triangular flow harmonics is observed to be very similar at different centralities after scaling the $v_{n}$ and $p_{\mathrm{T}}$ values by constant factors over the centrality interval $0-60$% and the $p_{\mathrm{T}}$ range $0.5 < p_{\mathrm{T}} < 5$ GeV.

==> HION-2016-06-PAPER-auxmat.tex <==
\section*{Auxiliary material}


\begin{figure}[h!]
\centering
\includegraphics[width=1\textwidth]{figaux_01}
\caption{
Correlation between the event-plane angles measured in the negative-$\eta$ 
  ($\Psi_n^{\mathrm{N}}$) and positive-$\eta$ ($\Psi_n^{\mathrm{P}}$) sides 
  of the FCal for harmonics $n$=2--7.
}
\label{fig:AUXpsinCorr}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{figaux_02}
\caption{
The \vn obtained with the EP method as a function of \pT, integrated over $|\eta|<2.5$. 
Each panel shows the resulta for a different centrality interval, 
  from most central in the top left panel to most peripheral in 
  the bottom right.\ 
For the \cent{0--0.1} and \cent{0--1} centrality intervals, only \vtwo--\vfive 
  are shown due to large statistical fluctuations for higher-order harmonics 
  \vsix and \vseven.\ 
Results are averaged over the intervals indicated by horizontal error bars.
The vertical error bars indicate statistical uncertainties.\
The shaded bands indicate systematic uncertainties.
}
\label{fig:AUXvnEPresults_pt}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{figaux_03}
\caption{
The \vn obtained with the EP method as a function of $\eta$, integrated over
  $0.8<\pT<1$~\GeV (left) ,$2<\pT<3$~\GeV (middle) and $7<\pT<60$~\GeV (right).\
From top to bottom each row shows the results for a different centrality interval: 
  0--0.1\%(top), 0--5\%, 10--20\%, 30--40\% and 60--70\%(bottom).\
Results are averaged over the intervals indicated by horizontal error bars.\
The vertical error bars indicate statistical uncertainties.\
The shaded bands indicate systematic uncertainties.
}
\label{fig:vnEP_eta}
\end{figure}


\begin{figure}[h!]
\includegraphics[width=0.9\linewidth]{figaux_04}
\caption{
The \vnep as a function of $N_{\mathrm{part}}$. 
Each panel shows the results for a different \pT interval.\ 
In the inset in the bottom right panel the \vsix and \vseven 
  integrated over $0.5<\pT<60~\GeV$ are replotted with an adjusted scale.\
Results are averaged over the intervals indicated by
  horizontal error bars.\
The vertical error bars indicate statistical uncertainties.\
The shaded bands indicate systematic uncertainties.
\label{fig:AUXvnEP_centrality}}
\end{figure}



\FloatBarrier

